Towards Autonomous Crop Monitoring: Inserting Sensors in Cluttered Environments

We present a contact-based phenotyping robot platform that can autonomously insert nitrate sensors into cornstalks to proactively monitor macronutrient levels in crops. This task is challenging because inserting such sensors requires sub-centimeter precision in an environment which contains high levels of clutter, lighting variation, and occlusion. To address these challenges, we develop a robust perception-action pipeline to detect and grasp stalks, and create a custom robot gripper which mechanically aligns the sensor before inserting it into the stalk. Through experimental validation on 48 unique stalks in a cornfield in Iowa, we demonstrate our platform's capability of detecting a stalk with 94% success, grasping a stalk with 90% success, and inserting a sensor with 60% success. In addition to developing an autonomous phenotyping research platform, we share key challenges and insights obtained from deployment in the field. Our research platform is open-sourced, with additional information available at https://kantor-lab.github.io/cornbot.

==> 7_2_deployment.tex <==

% \section{Data logging \& Deployment }~\label{sec:logger}
% \vspace{-10pt}

% %overview of 
% Once the sensor has been successfully inserted into the stalk, the robot deploys a datalogging unit near the stalk so that nitrate data can be monitored throughout the plant life cycle. As this is a research platform for a proof of concept, we limit the datalogging unit to monitor only one sensor, and the robot to deploy only up to five dataloggers before it needs to be manually reloaded.   

% The sensor samples the nitrate concentration of a corn stalk every five minutes over a 30 day period to monitor its health over the growth cycle. We created a deployable data logging unit that's compact, weather resistant, self-contained for power. The key components in the data logging unit are: arduino nano, custom ADC board, power boost board, and two 2800mAh batteries. To maximize the number of days in operation, we minimized the current draw by putting the Arduino on sleep-mode operation, which calculates to approximately 90 days of logging time.

% The datalogger deployment mechanism releases individual dataloggers to the ground near the corn once the sensor has been inserted. Each unit is housed in a slot where the bottom lid could be opened with individual servos that hooks to a latch. These latches can be opened/closed through either the serial commands on the PC or manually through the button pads on the side for quick manual access to the dataloggers. There were a couple design iterations on the deployment box to improve the wiring release mechanism as well as power efficiency. The first iteration had a wire management on coil setup to prevent tangling.

% However, although it did prevent tangling, the coil sometimes provided enough resistance so the datalogger would not fall out. We ended up removing the wire management into a coil, and instead just isolated wires from crossing into different cartridges as a simple workaround. Lastly, we modified the four bar link design to a latch mechanism in order to not draw power while its inactive. Without the latch, the servo would be drawing current to hold the boxes in place and would quickly deplete the external battery source.


% \subsection{Sensor calibration}

% These custom nitrate sensors require a calibration process to map nitrogen concentration (measured in PPM) to voltage. Each nitrate sensor leads to a unique mapping, which is why each sensor needs a calibration. The calibration process is done by measuring the voltage readings in two known concentration solutions: lower bound 200ppm and upper bound 2000 ppm. As the sensor takes time to stabilize, we take the average sample reading from 5 minute measurements, and then clean the sensor in a de-ionized 0 ppm solution before measuring in a different solution. As sensors readings in actual corn stalks yield ppm readings in between these lower and upper bounds, we can determine the nitrate reading of a corn from linear fitting a voltage measurement. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{images/calibration_sensor.jpg}
%     \caption{Custom nitrate sensor. Calibration procedure to map voltage readings to nitrate concentration in ppm.}
%     \label{fig:calibration}
%     \vspace{-10pt}
% \end{figure}
